A Kernel Perspective for Regularizing Deep Neural Networks

We propose a new point of view for regularizing deep neural networks by using the norm of a reproducing kernel Hilbert space (RKHS). Even though this norm cannot be computed, it admits upper and lower approximations leading to various practical strategies. Specifically, this perspective (i) provides a common umbrella for many existing regularization principles, including spectral norm and gradient penalties, or adversarial training, (ii) leads to new effective regularization penalties, and (iii) suggests hybrid strategies combining lower and upper bounds to get better approximations of the RKHS norm. We experimentally show this approach to be effective when learning on small datasets, or to obtain adversarially robust models.

==> discussion.tex <==
%!TEX root = main.tex

Making generic machine learning techniques more data efficient is crucial to
reduce the costs related to annotation. While other approaches may also be
important to solve this challenge, such as incorporating more prior
knowledge in the architecture~\citep[\eg,][]{oyallon2017scaling},
semi-supervised learning~\citep{chapelle06semi} or
meta-learning~\citep[when multiple tasks or datasets are available, see, \eg,][]{thrun1998lifelong},
basic regularization principles are needed.
Such principles are also essential for obtaining robust models in applications where
security is a concern, such as self-driving cars.
Our paper presents various algorithmic strategies for regularization on generic deep
convolutional networks, by leveraging the structure of an appropriate RKHS,
leading to many existing principles to regularization, as well as new effective variants,
in addition to providing theoretical guarantees and insights on different methods.


